TrABin: Trustworthy Analyses of Binaries

Verification of microkernels, device drivers, and crypto routines requires analyses at the binary level. In order to automate these analyses, in the last years several binary analysis platforms have been introduced. These platforms share a common design: the adoption of hardware-independent intermediate representations, a mechanism to translate architecture dependent code to this representation, and a set of architecture independent analyses that process the intermediate representation. The usage of these platforms to verify software introduces the need for trusting both the correctness of the translation from binary code to intermediate language (called transpilation) and the correctness of the analyses. Achieving a high degree of trust is challenging since the transpilation must handle (i) all the side effects of the instructions, (ii) multiple instruction encodings (e.g. ARM Thumb), and (iii) variable instruction length (e.g. Intel). Similarly, analyses can use complex transformations (e.g. loop unrolling) and simplifications (e.g. partial evaluation) of the artifacts, whose bugs can jeopardize correctness of the results. We overcome these problems by developing a binary analysis platform on top of the interactive theorem prover HOL4. First, we formally model a binary intermediate language and we prove correctness of several supporting tools (i.e. a type checker). Then, we implement two proof-producing transpilers, which respectively translate ARMv8 and CortexM0 programs to the intermediate language and generate a certificate. This certificate is a HOL4 proof demonstrating correctness of the translation. As demonstrating analysis, we implement a proof-producing weakest precondition generator, which can be used to verify that a given loop-free program fragment satisfies a contract. Finally, we use an AES encryption implementation to benchmark our platform.

==> benchmark.tex <==


The transpilation from binary code to $\bil$ is completely automatic and runs in two steps:
The first is the {\em transpiling step}, where each instruction is transpiled independently producing $\bil$ code and certificates; the second is the {\em merging step}, where we merge all the certificates deriving a single theorem aware of the program where the instructions run (i.e. jumps to other blocks). 
We successfully transpiled binary code compiled in a different of ways, with and without optimisation, compiled by us or found in binary form.
In the variety of software pieces to lift, we had chosen BLA due to their popularity and importance, libc, SQLite, lua, LIST.
The performance of the lifter for those binaries is shown in~Table~\ref{tbl:benchmark_lifting}.
\begin{table}[]
\caption{Timing of lifting instructions of popular binaries for ARMv8.}
\label{tbl:benchmark_lifting}
  \noindent\begin{center}
    \begin{tabular}{cccccc}
                                  &  Instructions & Transpiling step   & Merging step  & Total time  & Rate     \\ \hline
    lua                           &  37026        & 10917.170 s        & 6614.248  s   & 17531.418 s & 2.11 i/s \\
    SQLite                        &  61134        & 23734.919 s        & 16470.162 s   & 40205.081 s & 1.52 i/s \\
    libc                          &  23362        & 6264.500  s        & 2425.955  s   & 8690.455  s & 2.69 i/s \\ \hline
    \end{tabular}
  \end{center}
\end{table}
The lifter is optimised for small procedures to verify: This fact is reflected in the percentage of time spent in the merging step which increases with the number of instructions to lift.

Even if the tool is completely automatic, it relies on the completeness of the external model of the architecture.
This is required to produce the certificates for each instruction and the final certificate.
For this reason, we expect the lifter to fail to lift an instruction when this is not supported by the external model, i.e. the ARMv8 model does not support floating point operations.
Failure statistics are illustrated in~Table~\ref{tbl:benchmark_lifting_failures}.
\begin{table}[]
\caption{Failure rates of lifting instructions of popular binaries for ARMv8. Failures can be due to the {\em external model} or the tool itself.}
\label{tbl:benchmark_lifting_failures}
  \noindent\begin{center}
    \begin{tabular}{ccccc}
                                  & Instructions & Failed by model & Failed by lifter & Failed (total) \\ \hline
    lua                           & 37026        & 1161 (99.74\%)  & 3 (0.25\%)       & 1164           \\
    SQLite                        & 61134        & 2028 (98.68\%)  & 27 (1.31\%)      & 2055           \\
    libc                          & 23362        & 1404 (98.11\%)  & 27 (1.88\%)      & 1431           \\
    \end{tabular}
  \end{center}
\end{table}
As the reader can see, the tool work automatically and is able to transpile the very most of the binary code, apart from some rare cases {\color{red}of missing theorems (do we have better reasons?)}.
Failures can occur either because in the \textbf{external} model such instructions are not present, so no step theorem is provided to the lifter to work with, or because the lifter encounters a situation where {\color{red} good reason why it fails}.

The lifting part was extended with the optimisation of caching theorems related to the same instruction.
For example, lifting the $\mathit{nop}$ instruction is expected to be very frequent especially in optimised code.
So, the first time the $\mathit{nop}$ instruction will be a {\em miss} in the cache, and the lifter will need roughly half a second to produce the corresponding certificate.
All the successive times, the same instruction will be a {\em hit} in the cache, and the lifter will need roughly less than 3 milliseconds to retrieve the certificate from cache.
In summary, for cached instructions, the lifter is about 300 times faster.
The~Table~\ref{tbl:benchmark_lifting_most_cached} illustrates our benchmark on some of the lifted binaries showing that, for those binaries, the time spent to lift all of them would have been the same as lifting only 2, at most 3, of the same instruction without caching.
\begin{table}[htbp]
\caption{List of most cached instructions in lifted ARMv8 binaries lua, SQLite, and libc.}
\label{tbl:benchmark_lifting_most_cached}
  \noindent\begin{center}
    \begin{tabular}{clccc}
                                  & Instruction to lift                & Instructions & Hits \\ \hline
                                  & AA1303E0 (mov x0, x19)             &              & 1153 \\
    lua                           & D503201F (nop)                     & 37026        & 953  \\
                                  & D65F03C0 (ret)                     &              & 798  \\ \hline
                                  & D503201F (nop)                     &              & 975  \\
    SQLite                        & D65F03C0 (ret)                     & 61134        & 733  \\
                                  & A94153F3 (ldp x19, x20, [sp,\#16]) &              & 472  \\ \hline
                                  & D65F03C0 (ret)                     &              & 297  \\
    libc                          & D503201F (nop)                     & 23362        & 281  \\
                                  & A94153F3 (ldp x19, x20, [sp,\#16]) &              & 131  \\
    \end{tabular}
  \end{center}
\end{table}
To appreciate the colossal improvement in terms of efficiency due to caching technique, in~Table~\ref{tbl:benchmark_lifting_caching}  we split the whole set of lifted instructions in 4 subsets of equal size.
\begin{table}[htbp]
\caption{List of most cached instructions in lifted ARMv8 binaries lua, SQLite, and libc.}
\label{tbl:benchmark_lifting_caching}
  \noindent\begin{center}
    \begin{tabular}{ccc}
    Subset                   & Cache hits & Percentage of hits \\ \hline
    lua (1/4)                & 5084       & 54.92\%            \\
    lua (2/4)                & 5626       & 60.77\%            \\
    lua (3/4)                & 6688       & 72.24\%            \\
    lua (4/4)                & 6647       & 71.82\%            \\ \hline
    SQLite (1/4)             & 8064       & 52.76\%            \\
    SQLite (2/4)             & 10035      & 65.65\%            \\
    SQLite (3/4)             & 9651       & 63.14\%            \\
    SQLite (4/4)             & 10043      & 65.71\%            \\ \hline
    libc (1/4)               & 1990       & 34.06\%            \\
    libc (2/4)               & 2794       & 47.83\%            \\
    libc (3/4)               & 3002       & 51.39\%            \\
    libc (4/4)               & 3186       & 54.56\%            \\
    \end{tabular}
  \end{center}
\end{table}
Then, we reported the number of cache hits as a percentage of total instructions per subset.
As obviously expected, the number of cached instructions increases with the number of lifted instructions.
This trend renders the lifting slower at the beginning (when fewer hits occur) and faster at the end (where caching plays more a significant role).

Our aim is to create a tool which is automatic and relatively easy to be extended to other architectures.
This particular choice is based on the fact that we delegate the inspection of the binary code to the step theorem of the external model.
For this reason, our caching technique inherits the limitations provided by the step theorem.
We find that an example in this case is the best way to explain the concept.
Let us consider an instruction that adds the immediate number $3$ to register $\mathit{r1}$ and another that adds $4$ to $\mathit{r2}$.
The corresponding theorems look absolutely the same but for the two values.
So we could think of caching a {\em generic} theorem {\em for all} immediate numbers and registers, for that specific add operation.
Unfortunately, such granularity is impossible in our case, since we can {\em not} inspect the binary code, but only the output of the step theorem, which is {\em not} generic: If we did inspect the binary code, the tool would become much more platform dependent, and we would loose its ability to be easily extended to other architectures.
From another point of view, if using generic theorems was a choice, we would have pre-cached all the instructions, that is incorporating the whole model itself, letting the step theorem be totally useless, and the tool be totally architecture dependent.
Therefore, our caching technique cannot cache but the two instructions.
{\color{red} This limitation is visible in~Table~\ref{tbl:benckmark_cortexm0_caching}, where for the small set of instructions belonging to Cortex-M0, we would have quickly cached {\em all} the instructions.}

The generation of the weakest precondition is done in fragments of code to verify.
So the first operation to perform is to extract interesting fragments from the transpiled binary code.
Once we have a fragment of which compute the weakest precondition, it is performed in two steps:
In the first step COMPUTATION, and in the second step VARIABLE SUBSTITUTION.


OLD AND USELESS STUFF BELOW

A comparison of the time required to lift binary code in the two architectures (ARMv8 and Cortex-M0) is shown in~Table~\ref{tbl:benchmark_lifting_comparison_armv8_cortexm0}.
On average, we can see that the lifter from Cortex-M0 binaries performs faster than the lifter from ARMv8.
The reason of this difference is due to the simpler architecture of the former, i.e.\ smaller instruction set, therefore less theorems to handle.

The effect of caching some of the instructions can be seen from the time required to lift SOMETHING which is greater than the time required to lift SOMETHINGELSE.
In particular, the per-instruction time in the former is visibly lower than the latter, meaning that in the former the number of {\em hits} of instructions in cache was higher.


\begin{table}[]
\caption{Comparison}
\label{tbl:benchmark_lifting_comparison_armv8_cortexm0}
\begin{tabular}{rcccc}
                              &  Instructions & Failed (model) & Failed (lifter) & Failure rate \\ \hline
lua                           &  37026        & 10917.170 s & 6614.248  s & 2.11 i/s \\
SQLite                        &  61134        & 23734.919 s & 16470.162 s & 1.52 i/s \\
libc                          &  23362        & 6264.500  s & 2425.955  s & 2.69 i/s \\ \hline
 &                   &               &                &                            \\
\end{tabular}
\end{table}



\begin{table}[]
\caption{WP average timing}
\label{tbl:benchmark_wp_average}
\begin{tabular}{rlll}
                              &  Instructions  & ARMv8 & Cortex-M0 \\ \hline
Merging code                  &                &       &           \\
Checking for duplicate labels &                &       &           \\
Merging memory regions        &                &       &           \\ \hline
Total time                    &                &       &           \\
\end{tabular}
\end{table}

\begin{table}[]
\caption{WP timing for INTERESTING SOFTWARE (AES?)}
\label{tbl:benchmark_wp_software}
\begin{tabular}{rlll}
                              &  Instructions  & ARMv8 & Cortex-M0 \\ \hline
SOFTWARE1                     &                &       &           \\
SOFTWARE2                     &                &       &           \\
SOFTWARE3                     &                &       &           \\ \hline
Total time                    &                &       &           \\
\end{tabular}
\end{table}


We can see the same trend
in~Tables~\ref{tbl:benchmark_wp_average,tbl:benchmark_wp_software}
showing the weakest precondition transformer performance. 
%
%
%
%

